Adapters for Enhanced Modeling of Multilingual Knowledge and Text

Large language models appear to learn facts from the large text corpora they are trained on. Such facts are encoded implicitly within their many parameters, making it difficult to verify or manipulate what knowledge has been learned. Language models have recently been extended to multilingual language models (MLLMs), enabling knowledge to be learned across hundreds of languages. Meanwhile, knowledge graphs contain facts in an explicit triple format, which require careful and costly curation and are only available in a few high-resource languages, restricting their research and application. To address these issues, we propose to enhance MLLMs with knowledge from multilingual knowledge graphs (MLKGs) so as to tackle language and knowledge graph tasks across many languages, including low-resource ones. Specifically, we introduce a lightweight adapter set to enhance MLLMs with cross-lingual entity alignment and facts from MLKGs for many languages. Experiments on common benchmarks show that such enhancement benefits both MLLMs and MLKGs, achieving: (1) comparable or improved performance for knowledge graph completion and entity alignment relative to baselines, especially for low-resource languages (for which knowledge graphs are unavailable); and (2) improved MLLM performance on language understanding tasks that require multilingual factual knowledge; all while maintaining performance on other general language tasks.

==> main_text/orig_pre_carl/0abstract.tex <==
\begin{abstract}
Large pre-trained language models (LMs) and knowledge graphs (KGs) are typical knowledge sources for NLP tasks, which encode knowledge implicitly and explicitly\carl{Not v. clear; language models are `models' that have absorbed info from text data, KGs are `datasets', so this is grouping apples and oranges.}.
Recently, LMs have been extended to 
% multilingual scenarios, yielding 
multilingual LMs (MLLMs), enabling knowledge transfer across hundreds of languages. \carl{unclear sentence: is this trying to express that the information in different languages is not necessarily `aligned'?} However, the knowledge is encoded in a diffuse manner that is hard to manage. Meanwhile, KG research is limited to a few high-resource languages due to the cost of KG construction.
To address these problems, we propose to enhance MLLMs with the explicit knowledge of multilingual knowledge graphs (MLKGs) to be capable of tackling KG and language tasks across many languages, including those of low resource. Specifically, we introduce lightweight \textit{adapter set} into MLLMs to crystallize and integrate cross-lingual entity alignment and facts from MLKGs.
Experimental results on common benchmarks show that such integration of MLLMs and MLKGs benefits both, achieving: 
(1) comparable or improved performance than baselines for KG completion and entity alignment, especially for low-resource languages for which KGs are not available, which benefit from cross-lingual knowledge transfer; and (2) improving MLLM performance on language understanding tasks that require multilingual factual knowledge; while maintaining performance on other general language tasks.


\iffalse
Large pre-trained language models (LMs) and knowledge graphs (KGs) are typical knowledge sources for NLP tasks.
Recently, LMs have been extended to multilingual scenarios, yielding multilingual language models (MLLMs), enabling knowledge transfer between hundreds of languages. However, research on KGs is still limited to a few high-resource languages due to the high cost of KG construction.
In response to this problem, we propose to transfer the knowledge of multilingual knowledge graphs (MLKGs) across languages using MLLMs for automatic KG extension. Specifically, we design a set of lightweight knowledge adapters to integrate language-specific knowledge triples and cross-lingual entity alignments in MLKGs into MLLMs. %at both phrase and sentence levels.
Our experimental results on various benchmarks show that such integration of MLLMs and MLKGs is beneficial for both knowledge graph and language tasks: (1) our approach achieves comparable or better performance than approaches for KG completion and entity alignment, especially for low-resource and unseen languages, which benefit from the knowledge transfer ability of MLLMs; and (2) our approach improves the performance of MLLMs on language understanding tasks that require factual knowledge, and maintain performance on other general language tasks.


%In response to this problem, we propose to integrate multilingual LMs (MLLMs) and multilingual KGs (MLKGs) to benefit each other by:
%(1) transferring the knowledge of MLKGs from high-resource languages to low-resource languages using MLLMs for automatic KG extension; and (2) transferring the explicit knowledge from MLKGs to MLLMs for knowledge-intensive tasks.
%Specifically, we design four lightweight adapters to integrate the language-specific knowledge triples and cross-lingual entity alignments of MLKGs into MLLMs at both phrase and sentence levels.
%Experimental results on benchmarking MLKGs and MLLMs tasks show that our adapters: (1) outperform baseline methods on KG completion and entity alignment, especially for low-resource and unseen languages, which benefits from the knowledge transfer ability of MLLMs; and (2) improve the performance of MLLMs on language understanding tasks that require factual knowledge, and maintain the performance on the other general tasks. 
\fi
\end{abstract}

==> main_text/orig_pre_carl/1intro.tex <==
\section{Introduction}
%\mrinmaya{In my opinion, the below narrative is very indirect and not appropriate. I like the abstract. I think we should follow it to motivate the problem and then just be direct about what the model is: a knowledge-enhanced multilingual transformer (with adapters) with a combination mechanism which works for both KG tasks as well as language tasks; and we should talk about it. Again, we should have a nice figure of the model which describes the 4 objectives, their inputs and how the four adapters are then combined. Another figure which talks about the various training and finetuning stages. Question: Is this related to switch transformers and routing? How do I call your model?}
%\yifan{it's kind of similar to switch transformers. maybe we can call it knowledgeable adapter set? since our contribution is not about model design (we use AdapterFusion directly), calling LM+adapters with a new name might be confusing.}

% background: monolingual
% wenxiang: indirect and also duplicated in the paragraphs afterwards
%Language models (LMs) have achieved significant success across various natural language processing (NLP) tasks~\citep{devlin-etal-2019-bert,gpt_brown20}, which are pre-trained on a large corpus of web data and have been shown to contain rich knowledge implicitly in their parameters~\citep{petroni-etal-2019-language,rogers-etal-2020-primer}. 
%Knowledge graphs (KGs), which include rich facts about the world, provide effective knowledge basis for many NLP tasks such as entity linking~\citep{entitylinking_mulang20}, and question answering~\citep{kgqa_zhang22}.
%Recently, there are attempts that try to combine them for improvement. 
%\citet{kgbert_yao19} integrates the rich textual information of LMs to get entity embeddings, which helps to address the incompleteness issue of KGs.
%Various methods are proposed to enhance LMs with the explicit factual knowledge in KGs, where the performance of knowledge-intensive tasks is improved~\citep{zhang-etal-2019-ernie,wang-etal-2021-k}.
%Besides, \citet{sun-etal-2020-colake} proposes a method to get unified embeddings of both language and knowledge.

% wenxiang: issues of MLLMs and MLKGs
Pre-trained language models (LMs)~\citep{devlin-etal-2019-bert,gpt_brown20} and knowledge graphs (KGs) are two typical knowledge sources for current NLP tasks.
Pre-trained on plain texts, LMs have been successfully extended to multilingual LMs (MLLMs), where the knowledge is transferred across hundreds of languages~\citep{devlin-etal-2019-bert,xlm_conneau19,conneau-etal-2020-unsupervised}. However, as most neural systems, the knowledge in MLLMs is encoded in a diffused manner, which makes it difficult to interpret and utilize~\citep{lmkb_review_alKhamissi22}.
MLKGs require careful annotation of factual knowledge and cross-lingual entity alignments, making it prohibitively expensive to extend them to different languages.
Current open-source MLKGs such as WordNet~\citep{bond-foster-2013-linking} and Wikidata~\citep{wikidata_vrandevcic2014} suffer from incompleteness as a large number of knowledge triples and entity alignments are missing~\citep{mtranse_chen17,chen-etal-2020-multilingual}. Therefore, research on KGs is still limited to a few high-resource languages.


\begin{figure}[t!] 
	\centering
	\includegraphics[width = 0.95\columnwidth]{./figures/mlkg.pdf}
	\vspace{-.31cm}
	\caption{Combining MLLMs and MLKGs benefits each other. MLKGs suffer from incompleteness. MLLMs can help to find missing alignments and triples. When MLLMs do knowledge-intensive tasks such as relation classification, using the explicit knowledge in MLKGs is also helpful.} % For example, the entity \textit{Nonfiction} is not aligned with its Italian label \textit{Saggistica}, and the knowledge triple \textit{(Alain de Boon, lives in, Switzerland)} is missing in Chinese and Italian. 
	\vspace{-.6cm}
	\label{fig:compare}
\end{figure}

In this work, we propose to overcome these limitations by transferring the knowledge of MLKGs from high-resource languages to low-resource languages using MLLMs.
Combining both can also transfer the explicit knowledge from MLKGs to MLLMs for knowledge-intensive language tasks, which is one of the key challenges in MLLMs~\citep{lmkb_review_alKhamissi22}.
%
While this idea seems intuitive,  there is no easy way to combine the generalizability of MLLMs and the explicit knowledge of MLKGs.
Existing KI methods utilize LMs and KGs in two different ways by: (1) training KG embeddings and LMs individually, and aggregating them correspondingly for the linked entities in sentences~\citep{peters-etal-2019-knowledge,zhang-etal-2019-ernie}; or (2) injecting the KG knowledge into LMs' parameters with joint training~\citep{kbert_liu19,wang-etal-2021-k}. 
The first method needs to embed entity labels in KGs and accurately extract entities in sentences which is unrealistic for hundreds of languages. The second method typically suffers from the \textit{curse of multilinguality}~\citep{conneau-etal-2020-unsupervised,mllmcurse_doddapaneni21} and \textit{catastrophic forgetting}~\citep{forgetting_kirkpatrick16} due to limited model capacity. 
Most importantly, both methods integrate knowledge implicitly, which makes it difficult to access the knowledge for the KG extension~\citep{lmkb_review_alKhamissi22}.
%
Regarding the lack of a multilingual KI corpus, \citet{mlkidamo_liu21} propose to synthesize code-switched sentences as the KI data. However, they achieve negligible improvements with their MLKG-enhanced MLLMs since they do not address the other issues stated above.

%\textbf{Existing knowledge integration (KI) methods}~\citep{peters-etal-2019-knowledge,zhang-etal-2019-ernie,kbert_liu19,wang-etal-2021-k} still integrate knowledge in an implicit way, which are not interpretable and the knowledge is hard to access for the MLKG extension. Besides, they are dedicated for monolingual LMs and are unsuitable in multilingual scenarios due to their limited designs and the lack of multilingual KI corpus.
%Data is another bottleneck for KI in the multilingual setting. The text in KGs are phrases such as entity labels and relation labels, while text fed into LMs is usually longer (sentences or paragraphs). 


To address above challenges, we propose a set of lightweight (i.e., the size of adapter is $0.5\%$ of MLLMs) knowledge adapters to enhance MLLMs with MLKGs in an interpretable way. 
Our adapter set is designed to crystallize and integrate the knowledge \textbf{T}riples and cross-lingual \textbf{E}ntity alignments at both \textbf{P}hrase and \textbf{S}entence levels from MLKGs in MLLMs, leading to four modules (Adapter-EP/TP/ES/TS).
They are trained individually to enhance different kinds of knowledge into the geometry properties of MLLM representations using the MLKG embedding objective~\citep{mtranse_chen17}, and their outputs are aggregated by a fusion mechanism to combine the knowledge~\citep{pfeiffer-etal-2021-adapterfusion} for downstream tasks.

We conduct experiments on various downstream tasks to demonstrate the effectiveness of our approach.
For MLKG tasks, our method obtains comparable performance to existing baselines on the KG completion benchmark, and significantly better performance on the entity alignment benchmark. 
More importantly, we extend the test set with low-resource (or unseen) languages, on which our method achieves promising results as on those high-resource languages. The improvements over base MLLMs are always significant.
It demonstrates that our method can adapt the knowledge generalizability of MLLMs to MLKGs for better KG extension.
As for MLLM tasks, our method improve existing MLLMs noticeably on knowledge-intensive tasks such as cross-lingual relation classification, which indicates the effectiveness of explicit knowledge, and maintain the performance on general language tasks such as NER and QA.


%wxjiao{However, the knowledge (i.e., factual knowledge and cross-lingual knowledge) is encoded in a diffused manner, making it uninterpretable and difficult to be used for knowledge-intensive language tasks~\citep{lmkb_review_alKhamissi22}. On the other hand, KGs provide explicit factual knowledge but require careful annotation, making them prohibitively expensive to scale into different languages. Particularly, open-sourced multilingual KGs~(MLKGs) such as WordNet~\citep{bond-foster-2013-linking} and Wikidata~\citep{wikidata_vrandevcic2014} often suffer from the incompleteness issues such that a fairly large number of knowledge triples and entity alignments are missing~\citep{mtranse_chen17,chen-etal-2020-multilingual}. Therefore, researches on KGs are still limited in a few high-resource languages. In this work, we propose to combine the generalizability of MLLMs and the explicit knowledge of MLKGs to address the above issues, which has been barely explored before.}




%% monolingual -> multilingual
%In the multilingual scenario, the development of LMs and KGs is also carried out at the same time.
% MLLM: pros and cons + KI (damo) and probe (universal space)
%Multilingual LMs (MLLMs), based on the powerful generalizability, have achieved significant success on the knowledge transfer across hundreds of languages~\citep{devlin-etal-2019-bert,xlm_conneau19,conneau-etal-2020-unsupervised}. 
%However, similar to monolingual LMs, the knowledge (factual knowledge and cross-lingual knowledge) is encoded in a diffused manner, which makes it hard to be interpreted and used~\citep{lmkb_review_alKhamissi22}.
%% MLKG
%Multilingual knowledge graphs (MLKGs), such as WordNet~\citep{bond-foster-2013-linking} and Wikidata~\citep{wikidata_vrandevcic2014}, contain explicit knowledge about facts and cross-lingual alignments across a large number of languages.
%However, as most monolingual KGs, it suffers from incompleteness, and a fairly large number of knowledge triples and entity alignments are missing~\citep{mtranse_chen17}. 
%% issue
%Intuitively, we can also combine the generalizability of MLLMs and the explicit knowledge of MLKGs to address their issues. But, we argue that there are many problems if simply extending existing methods to the multilingual scenario.

%\wxjiao{Existing knowledge integration (KI) methods dedicated for monolingual LMs and KGs are unsuitable for the multilingual scenarios due to their non-extensive model designs and lack of alignments in multilingual corpus. KI methods utilize LMs and KGs in two different ways by: (1) training KG embeddings and LMs individually, and aggregating them correspondingly for the linked entities in sentences~\citep{peters-etal-2019-knowledge,zhang-etal-2019-ernie}; or (2) injecting the KG knowledge into LMs' parameters with joint training~\citep{kbert_liu19,wang-etal-2021-k}. The first method needs to embed all entities in KGs and accurately extract entities in sentences, which becomes unrealistic for the significantly increased entities in hundreds of languages. The second method may suffer from the \textit{curse of multilinguality}~\citep{conneau-etal-2020-unsupervised,mllmcurse_doddapaneni21} and \textit{catastrophic forgetting}~\citep{forgetting_kirkpatrick16} due to the limited model capacity. Most importantly, both methods do not take into account the alignment information in MLKGs, which limits the knowledge transfer between KGs in different languages.}


%\yifan{we can put below paragraphs to a new section}
%% KI not work: LM
%There are two types of knowledge integration (KI) methods for monolingual LMs.
%First, entities in KGs are first embedded, and LMs integrating knowledge by aggregating the external embeddings with their representations of the linked entities in sentences~\citep{peters-etal-2019-knowledge,zhang-etal-2019-ernie}. This kind of KI methods need to embed all entities in KGs and accurately extract entities in sentences. 
%However, for the multilingual setting, the size of external embeddings could be much larger with entities in hundreds of languages. It is also unrealistic to extract entities accurately for all languages. Besides, aggregating entity embedding can only integrate factual knowledge, where the cross-lingual alignments in MLKGs are totally ignored. 
%Second, KI can be done by integrating knowledge into model parameters~\citep{kbert_liu19,wang-etal-2021-k}.
%However, different from monolingual LMs, MLLMs suffer from the \textit{curse of multilinguality}~\citep{conneau-etal-2020-unsupervised,mllmcurse_doddapaneni21}. The limited model capacity prevent them from learning new knowledge, and simply integrating new knowledge of MLKGs would cause catastrophic forgetting of already learned knowledge~\citep{forgetting_kirkpatrick16}.
%Even if modules with new parameters can be introduced and trained to capture knowledge~\citep{he-etal-2020-bert,wang-etal-2021-k}, it is still difficult to integrate knowledge about facts and cross-lingual entity alignments at a same time.

%\wxjiao{% wenxiang: data bottleneck and related baseline
%Data is also a bottleneck for KI in multilingual scenarios. The text in KGs are phrases such as entity labels and relation labels, while the text fed into LMs is usually sentences. It is unrealistic to annotate alignments between sentences and knowledge triples, or verbalize such large number of triples by writing prompt templates for hundreds of languages. Even though \citet{mlkidamo_liu21} propose to synthesize the code-switched sentences as the KI data, they achieve negligible improvements with their MLKG-enhanced MLLMs since they do not address the other issues stated above. } 


%% general difficulty
%Besides, the KI data could be the bottleneck. The text in KGs are phrases such as entity labels and relation labels, while the text fed into LMs is usually sentences. It is unrealistic to annotate alignments between sentences and knowledge triples, or verbalize such large number of triples by writing prompt templates for hundreds of languages.
%% existing work
%Even if \citet{mlkidamo_liu21} propose to use the code switched synthetic sentences for generating the KI data, as they do not address other issues, there is no obvious improvement on their MLKG-enhanced MLLMs. %% we have comparison experiment with their model 


%\wxjiao{% wenxiang: ours
%To address these issues, we propose a set of knowledgeable adapters to enhance MLLMs with MLKGs in an interpretable way.  Our adapter set is designed to model the knowledge \textbf{T}riples and cross-lingual \textbf{E}ntity alignments at both \textbf{P}hrase and \textbf{S}entence levels, which naturally includes \textbf{Adapter-EP}, \textbf{Adapter-TP}, \textbf{Adapter-ES} and \textbf{Adapter-TS}. {\color{red} Brief the training pipeline of adapters.} The four adapters are aggregated by a fusion mechanism~\citep{pfeiffer-etal-2021-adapterfusion} to perform downstream tasks. We conduct experiments on downstream tasks of MLKGs and MLLMs to demonstrate the effectiveness of our adapters. For MLKG tasks, our method can obtain good performance as existing baselines on the MLKG completion benchmark, and significantly better performance on the entity alignment benchmark.  More importantly, we extend the test set with 20 low-resource (or unseen) languages, on which our method achieves promising results as on those high-resource languages.  It demonstrates that our method can adapt the knowledge generalizability of MLLMs to MLKGs for better KG extension. As for MLLMs tasks, our method can improve existing MLLMs on knowledge-intensive tasks, which indicates the effectiveness of explicit knowledge, and maintain the performance on general language tasks.}



% contribution
%Therefore, in this paper, to address above issues, we propose a set of knowledgeable adapters to use MLKG to enhance MLLM in an interpretable way. The enhanced MLLM combines the properties of LM's generalizability and KG's explicit, which can perform good on both KG tasks (e.g., MLKG completion) and LM tasks (e.g., cross-lingual relation extraction).
%There are four adapters with a fusion mechanism~\citep{pfeiffer-etal-2021-adapterfusion} to encode factual knowledge and cross-lingual knowledge in both phrase-level and sentence-level.
%% exp
%In our experiments, we find that for the KG tasks, our method can achieve better performance as existing baselines on the MLKG completion benchmark, and significantly better performance on the entity alignment benchmark. Beside, we extend the test set with $20$ low-resource languages, and find that our method is capable of using the powerful generalizability of LMs and achieve comparable performance for them under the zero-shot setting.
%From the MLLM side, our method can improve existing MLLMs on knowledge-intensive tasks, and keep the performance on the general MLLM tasks.

